Obtaining Smoothly Navigable Approximation Sets in Bi-Objective Multi-Modal Optimization

Even if a Multi-modal Multi-Objective Evolutionary Algorithm (MMOEA) is designed to find solutions well spread over all locally optimal approximation sets of a Multi-modal Multi-objective Optimization Problem (MMOP), there is a risk that the found set of solutions is not smoothly navigable because the solutions belong to various niches, reducing the insight for decision makers. To tackle this issue, a new MMOEAs is proposed: the Multi-Modal B\'ezier Evolutionary Algorithm (MM-BezEA), which produces approximation sets that cover individual niches and exhibit inherent decision-space smoothness as they are parameterized by B\'ezier curves. MM-BezEA combines the concepts behind the recently introduced BezEA and MO-HillVallEA to find all locally optimal approximation sets. When benchmarked against the MMOEAs MO_Ring_PSO_SCD and MO-HillVallEA on MMOPs with linear Pareto sets, MM-BezEA was found to perform best in terms of best hypervolume.

==> sections/BASE_TEMPLATE.tex <==
ACM's consolidated article template, introduced in 2017, provides a
consistent \LaTeX\ style for use across ACM publications, and
incorporates accessibility and metadata-extraction functionality
necessary for future Digital Library endeavors. Numerous ACM and
SIG-specific \LaTeX\ templates have been examined, and their unique
features incorporated into this single new template.

If you are new to publishing with ACM, this document is a valuable
guide to the process of preparing your work for publication. If you
have published with ACM before, this document provides insight and
instruction into more recent changes to the article template.

The ``\verb|acmart|'' document class can be used to prepare articles
for any ACM publication --- conference or journal, and for any stage
of publication, from review to final ``camera-ready'' copy, to the
author's own version, with {\itshape very} few changes to the source.

\section{Template Overview}
As noted in the introduction, the ``\verb|acmart|'' document class can
be used to prepare many different kinds of documentation --- a
double-blind initial submission of a full-length technical paper, a
two-page SIGGRAPH Emerging Technologies abstract, a ``camera-ready''
journal article, a SIGCHI Extended Abstract, and more --- all by
selecting the appropriate {\itshape template style} and {\itshape
  template parameters}.

This document will explain the major features of the document
class. For further information, the {\itshape \LaTeX\ User's Guide} is
available from
\url{https://www.acm.org/publications/proceedings-template}.

\subsection{Template Styles}

The primary parameter given to the ``\verb|acmart|'' document class is
the {\itshape template style} which corresponds to the kind of publication
or SIG publishing the work. This parameter is enclosed in square
brackets and is a part of the {\verb|documentclass|} command:
\begin{verbatim}
  \documentclass[STYLE]{acmart}
\end{verbatim}

Journals use one of three template styles. All but three ACM journals
use the {\verb|acmsmall|} template style:
\begin{itemize}
\item {\verb|acmsmall|}: The default journal template style.
\item {\verb|acmlarge|}: Used by JOCCH and TAP.
\item {\verb|acmtog|}: Used by TOG.
\end{itemize}

The majority of conference proceedings documentation will use the {\verb|acmconf|} template style.
\begin{itemize}
\item {\verb|acmconf|}: The default proceedings template style.
\item{\verb|sigchi|}: Used for SIGCHI conference articles.
\item{\verb|sigchi-a|}: Used for SIGCHI ``Extended Abstract'' articles.
\item{\verb|sigplan|}: Used for SIGPLAN conference articles.
\end{itemize}

\subsection{Template Parameters}

In addition to specifying the {\itshape template style} to be used in
formatting your work, there are a number of {\itshape template parameters}
which modify some part of the applied template style. A complete list
of these parameters can be found in the {\itshape \LaTeX\ User's Guide.}

Frequently-used parameters, or combinations of parameters, include:
\begin{itemize}
\item {\verb|anonymous,review|}: Suitable for a ``double-blind''
  conference submission. Anonymizes the work and includes line
  numbers. Use with the \verb|\acmSubmissionID| command to print the
  submission's unique ID on each page of the work.
\item{\verb|authorversion|}: Produces a version of the work suitable
  for posting by the author.
\item{\verb|screen|}: Produces colored hyperlinks.
\end{itemize}

This document uses the following string as the first command in the
source file:
\begin{verbatim}
\documentclass[sigconf]{acmart}
\end{verbatim}

\section{Modifications}

Modifying the template --- including but not limited to: adjusting
margins, typeface sizes, line spacing, paragraph and list definitions,
and the use of the \verb|\vspace| command to manually adjust the
vertical spacing between elements of your work --- is not allowed.

{\bfseries Your document will be returned to you for revision if
  modifications are discovered.}

\section{Typefaces}

The ``\verb|acmart|'' document class requires the use of the
``Libertine'' typeface family. Your \TeX\ installation should include
this set of packages. Please do not substitute other typefaces. The
``\verb|lmodern|'' and ``\verb|ltimes|'' packages should not be used,
as they will override the built-in typeface families.

\section{Title Information}

The title of your work should use capital letters appropriately -
\url{https://capitalizemytitle.com/} has useful rules for
capitalization. Use the {\verb|title|} command to define the title of
your work. If your work has a subtitle, define it with the
{\verb|subtitle|} command.  Do not insert line breaks in your title.

If your title is lengthy, you must define a short version to be used
in the page headers, to prevent overlapping text. The \verb|title|
command has a ``short title'' parameter:
\begin{verbatim}
  \title[short title]{full title}
\end{verbatim}

\section{Authors and Affiliations}

Each author must be defined separately for accurate metadata
identification. Multiple authors may share one affiliation. Authors'
names should not be abbreviated; use full first names wherever
possible. Include authors' e-mail addresses whenever possible.

Grouping authors' names or e-mail addresses, or providing an ``e-mail
alias,'' as shown below, is not acceptable:
\begin{verbatim}
  \author{Brooke Aster, David Mehldau}
  \email{dave,judy,steve@university.edu}
  \email{firstname.lastname@phillips.org}
\end{verbatim}

The \verb|authornote| and \verb|authornotemark| commands allow a note
to apply to multiple authors --- for example, if the first two authors
of an article contributed equally to the work.

If your author list is lengthy, you must define a shortened version of
the list of authors to be used in the page headers, to prevent
overlapping text. The following command should be placed just after
the last \verb|\author{}| definition:
\begin{verbatim}
  \renewcommand{\shortauthors}{McCartney, et al.}
\end{verbatim}
Omitting this command will force the use of a concatenated list of all
of the authors' names, which may result in overlapping text in the
page headers.

The article template's documentation, available at
\url{https://www.acm.org/publications/proceedings-template}, has a
complete explanation of these commands and tips for their effective
use.

Note that authors' addresses are mandatory for journal articles.

\section{Rights Information}

Authors of any work published by ACM will need to complete a rights
form. Depending on the kind of work, and the rights management choice
made by the author, this may be copyright transfer, permission,
license, or an OA (open access) agreement.

Regardless of the rights management choice, the author will receive a
copy of the completed rights form once it has been submitted. This
form contains \LaTeX\ commands that must be copied into the source
document. When the document source is compiled, these commands and
their parameters add formatted text to several areas of the final
document:
\begin{itemize}
\item the ``ACM Reference Format'' text on the first page.
\item the ``rights management'' text on the first page.
\item the conference information in the page header(s).
\end{itemize}

Rights information is unique to the work; if you are preparing several
works for an event, make sure to use the correct set of commands with
each of the works.

The ACM Reference Format text is required for all articles over one
page in length, and is optional for one-page articles (abstracts).

\section{CCS Concepts and User-Defined Keywords}

Two elements of the ``acmart'' document class provide powerful
taxonomic tools for you to help readers find your work in an online
search.

The ACM Computing Classification System ---
\url{https://www.acm.org/publications/class-2012} --- is a set of
classifiers and concepts that describe the computing
discipline. Authors can select entries from this classification
system, via \url{https://dl.acm.org/ccs/ccs.cfm}, and generate the
commands to be included in the \LaTeX\ source.

User-defined keywords are a comma-separated list of words and phrases
of the authors' choosing, providing a more flexible way of describing
the research being presented.

CCS concepts and user-defined keywords are required for for all
articles over two pages in length, and are optional for one- and
two-page articles (or abstracts).

\section{Sectioning Commands}

Your work should use standard \LaTeX\ sectioning commands:
\verb|section|, \verb|subsection|, \verb|subsubsection|, and
\verb|paragraph|. They should be numbered; do not remove the numbering
from the commands.

Simulating a sectioning command by setting the first word or words of
a paragraph in boldface or italicized text is {\bfseries not allowed.}

\section{Tables}

The ``\verb|acmart|'' document class includes the ``\verb|booktabs|''
package --- \url{https://ctan.org/pkg/booktabs} --- for preparing
high-quality tables.

Table captions are placed {\itshape above} the table.

Because tables cannot be split across pages, the best placement for
them is typically the top of the page nearest their initial cite.  To
ensure this proper ``floating'' placement of tables, use the
environment \textbf{table} to enclose the table's contents and the
table caption.  The contents of the table itself must go in the
\textbf{tabular} environment, to be aligned properly in rows and
columns, with the desired horizontal and vertical rules.  Again,
detailed instructions on \textbf{tabular} material are found in the
\textit{\LaTeX\ User's Guide}.

Immediately following this sentence is the point at which
Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed output of
this document.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

To set a wider table, which takes up the whole width of the page's
live area, use the environment \textbf{table*} to enclose the table's
contents and the table caption.  As with a single-column table, this
wide table will ``float'' to a location deemed more
desirable. Immediately following this sentence is the point at which
Table~\ref{tab:commands} is included in the input file; again, it is
instructive to compare the placement of the table here with the table
in the printed output of this document.

\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}

Always use midrule to separate table header rows from data rows, and
use it only for this purpose. This enables assistive technologies to
recognise table headers and support their users in navigating tables
more easily.

\section{Math Equations}
You may want to display math equations in three distinct styles:
inline, numbered or non-numbered display.  Each of the three are
discussed in the next sections.

\subsection{Inline (In-text) Equations}
A formula that appears in the running text is called an inline or
in-text formula.  It is produced by the \textbf{math} environment,
which can be invoked with the usual
\texttt{{\char'134}begin\,\ldots{\char'134}end} construction or with
the short form \texttt{\$\,\ldots\$}. You can use any of the symbols
and structures, from $\alpha$ to $\omega$, available in
\LaTeX~\cite{Lamport:LaTeX}; this section will simply show a few
examples of in-text equations in context. Notice how this equation:
\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},
set here in in-line math style, looks slightly different when
set in display style.  (See next section).

\subsection{Display Equations}
A numbered display equation---one set off by vertical space from the
text and centered horizontally---is produced by the \textbf{equation}
environment. An unnumbered display equation is produced by the
\textbf{displaymath} environment.

Again, in either environment, you can use any of the symbols and
structures available in \LaTeX\@; this section will just give a couple
of examples of display equations in context.  First, consider the
equation, shown as an inline equation above:
\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}
Notice how it is formatted somewhat differently in
the \textbf{displaymath}
environment.  Now, we'll enter an unnumbered equation:
\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}
and follow it with another numbered equation:
\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}
just to demonstrate \LaTeX's able handling of numbering.

\section{Figures}

The ``\verb|figure|'' environment should be used for figures. One or
more images can be placed within a figure. If your figure contains
third-party material, you must clearly identify it as such, as shown
in the example below.
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{sample-franklin}
  \caption{1907 Franklin Model D roadster. Photograph by Harris \&
    Ewing, Inc. [Public domain], via Wikimedia
    Commons. (\url{https://goo.gl/VLCRBB}).}
  \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}

Your figures should contain a caption which describes the figure to
the reader.

Figure captions are placed {\itshape below} the figure.

Every figure should also have a figure description unless it is purely
decorative. These descriptions convey what’s in the image to someone
who cannot see it. They are also used by search engine crawlers for
indexing images, and when images cannot be loaded.

A figure description must be unformatted plain text less than 2000
characters long (including spaces).  {\bfseries Figure descriptions
  should not repeat the figure caption – their purpose is to capture
  important information that is not already provided in the caption or
  the main text of the paper.} For figures that convey important and
complex new information, a short text description may not be
adequate. More complex alternative descriptions can be placed in an
appendix and referenced in a short figure description. For example,
provide a data table capturing the information in a bar chart, or a
structured list representing a graph.  For additional information
regarding how best to write figure descriptions and why doing this is
so important, please see
\url{https://www.acm.org/publications/taps/describing-figures/}.

\subsection{The ``Teaser Figure''}

A ``teaser figure'' is an image, or set of images in one figure, that
are placed after all author and affiliation information, and before
the body of the article, spanning the page. If you wish to have such a
figure in your article, place the command immediately before the
\verb|\maketitle| command:
\begin{verbatim}
  \begin{teaserfigure}
    \includegraphics[width=\textwidth]{sampleteaser}
    \caption{figure caption}
    \Description{figure description}
  \end{teaserfigure}
\end{verbatim}

\section{Citations and Bibliographies}

The use of \BibTeX\ for the preparation and formatting of one's
references is strongly recommended. Authors' names should be complete
--- use full first names (``Donald E. Knuth'') not initials
(``D. E. Knuth'') --- and the salient identifying features of a
reference should be included: title, year, volume, number, pages,
article DOI, etc.

The bibliography is included in your source document with these two
commands, placed just before the \verb|\end{document}| command:
\begin{verbatim}
  \bibliographystyle{ACM-Reference-Format}
  \bibliography{bibfile}
\end{verbatim}
where ``\verb|bibfile|'' is the name, without the ``\verb|.bib|''
suffix, of the \BibTeX\ file.

Citations and references are numbered by default. A small number of
ACM publications have citations and references formatted in the
``author year'' style; for these exceptions, please include this
command in the {\bfseries preamble} (before the command
``\verb|\begin{document}|'') of your \LaTeX\ source:
\begin{verbatim}
  \citestyle{acmauthoryear}
\end{verbatim}

  Some examples.  A paginated journal article \cite{Abril07}, an
  enumerated journal article \cite{Cohen07}, a reference to an entire
  issue \cite{JCohen96}, a monograph (whole book) \cite{Kosiur01}, a
  monograph/whole book in a series (see 2a in spec. document)
  \cite{Harel79}, a divisible-book such as an anthology or compilation
  \cite{Editor00} followed by the same example, however we only output
  the series if the volume number is given \cite{Editor00a} (so
  Editor00a's series should NOT be present since it has no vol. no.),
  a chapter in a divisible book \cite{Spector90}, a chapter in a
  divisible book in a series \cite{Douglass98}, a multi-volume work as
  book \cite{Knuth97}, a couple of articles in a proceedings (of a
  conference, symposium, workshop for example) (paginated proceedings
  article) \cite{Andler79, Hagerup1993}, a proceedings article with
  all possible elements \cite{Smith10}, an example of an enumerated
  proceedings article \cite{VanGundy07}, an informally published work
  \cite{Harel78}, a couple of preprints \cite{Bornmann2019,
    AnzarootPBM14}, a doctoral dissertation \cite{Clarkson85}, a
  master's thesis: \cite{anisi03}, an online document / world wide web
  resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game
  (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03} and \cite{Lee05}
  and (Case 3) a patent \cite{JoeScientist001}, work accepted for
  publication \cite{rous08}, 'YYYYb'-test for prolific author
  \cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might
  contain 'duplicate' DOI and URLs (some SIAM articles)
  \cite{Kirschmer:2010:AEI:1958016.1958018}. Boris / Barbara Beeton:
  multi-volume works as books \cite{MR781536} and \cite{MR781537}. A
  couple of citations with DOIs:
  \cite{2004:ITE:1009386.1010128,Kirschmer:2010:AEI:1958016.1958018}. Online
  citations: \cite{TUGInstmem, Thornburg01, CTANacmart}. Artifacts:
  \cite{R} and \cite{UMassCitations}.

\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

\section{Appendices}

If your work needs an appendix, add it before the
``\verb|\end{document}|'' command at the conclusion of your source
document.

Start the appendix with the ``\verb|appendix|'' command:
\begin{verbatim}
  \appendix
\end{verbatim}
and note that in the appendix, sections are lettered, not
numbered. This document has two appendices, demonstrating the section
and subsection identification method.

\section{SIGCHI Extended Abstracts}

The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
not in Word) produces a landscape-orientation formatted article, with
a wide left margin. Three environments are available for use with the
``\verb|sigchi-a|'' template style, and produce formatted output in
the margin:
\begin{itemize}
\item {\verb|sidebar|}:  Place formatted text in the margin.
\item {\verb|marginfigure|}: Place a figure in the margin.
\item {\verb|margintable|}: Place a table in the margin.
\end{itemize}

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
\begin{acks}
To Robert, for the bagels and explaining CMYK and color spaces.
\end{acks}

\bibliographystyle{ACM-Reference-Format}
\bibliography{sample-base}

%%
%% If your work has an appendix, this is the place to put it.
\appendix

\section{Research Methods}

\subsection{Part One}

Lorem ipsum dolor sit amet, consectetur adipiscing elit. Morbi
malesuada, quam in pulvinar varius, metus nunc fermentum urna, id
sollicitudin purus odio sit amet enim. Aliquam ullamcorper eu ipsum
vel mollis. Curabitur quis dictum nisl. Phasellus vel semper risus, et
lacinia dolor. Integer ultricies commodo sem nec semper.

\subsection{Part Two}

Etiam commodo feugiat nisl pulvinar pellentesque. Etiam auctor sodales
ligula, non varius nibh pulvinar semper. Suspendisse nec lectus non
ipsum convallis congue hendrerit vitae sapien. Donec at laoreet
eros. Vivamus non purus placerat, scelerisque diam eu, cursus
ante. Etiam aliquam tortor auctor efficitur mattis.

\section{Online Resources}

Nam id fermentum dui. Suspendisse sagittis tortor a nulla mollis, in
pulvinar ex pretium. Sed interdum orci quis metus euismod, et sagittis
enim maximus. Vestibulum gravida massa ut felis suscipit
congue. Quisque mattis elit a risus ultrices commodo venenatis eget
dui. Etiam sagittis eleifend elementum.

Nam interdum magna at lectus dignissim, ac dignissim lorem
rhoncus. Maecenas eu arcu ac neque placerat aliquam. Nunc pulvinar
massa et mattis lacinia.

==> sections/acknowledge.tex <==
\begin{acks}
    Leah R.M. Dickhoff was supported by the Dutch Cancer Society (\grantsponsor{0}{KWF kankerbestrijding}{https://www.kwf.nl/}, Project N.\grantnum{0}{12183}) and \grantsponsor{1}{Elekta}{https://www.elekta.com/}.
\end{acks} 

==> sections/set-bezea-linkage-tree.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[
    level/.style={sibling distance=35mm/#1},
    text=!50!black,
    >=latex,
    font=\sffamily
    ]

\node (z){$C_{q,b} \colon \left\{x_0, x_1, ..., x_7\right\}$} 
  child {node (a) {$C_q^0 \colon \left\{x_0, x_1, x_2, x_3\right\}$}
    child {node  (b) {$\left\{x_0, x_2\right\}$}[no edge from this parent]
      %child {node (b1) {$x_0$}}
      %child {node (b2) {$x_1$}}
    }
    child {node (g) {$\left\{x_1, x_3\right\}$}[no edge from this parent]
      %child {node (g1) {$x_2$}}
      %child {node (g2) {$x_3$}}
    }
  }
    child {node (d) {$C_q^1 \colon \left\{x_4, x_5, x_6, x_7\right\}$}
      child {node  (e) {$\left\{x_4, x_6\right\}$}[no edge from this parent]
          %child {node (e1) {$x_4$}}
          %child {node (e2) {$x_5$}}
      }
      child {node (f) {$\left\{x_5, x_7\right\}$}[no edge from this parent]
          %child {node (f1) {$x_6$}}
          %child {node (f2) {$x_7$}}
  }
};

\node[left=2 of z]  (ln1) {}[no edge from this parent]
    child {node (ln2) {}[no edge from this parent]
        child {node (ln3) {}[no edge from this parent]}};
\draw [!70!black,thick,decorate, decoration = {calligraphic brace}] (ln2.north west) --node[midway,left]{Level 2 \hspace{2em}}(ln1.west);
\draw [!70!black,thick,decorate, decoration = {calligraphic brace}] (ln3.west) --node[midway,left]{Level 1  \hspace{2em}} (ln2.south west);


%\draw[blue!70!black,thick]  (b.south) -- (g1.north); 
%\draw[blue!70!black,thick]  (b.south) -- (b1.north);
%\draw[blue!70!black,thick]  (g.south) -- (b2.north);
%\draw[blue!70!black,thick]  (g.south) -- (g2.north);

%\draw[blue!70!black,thick]  (e.south) -- (e1.north); 
%\draw[blue!70!black,thick]  (e.south) -- (f1.north);
%\draw[blue!70!black,thick]  (f.south) -- (e2.north);
%\draw[blue!70!black,thick]  (f.south) -- (f2.north);

% Separate control points
%\draw[dashed,rounded corners=10]($(b1) + (-.25,.3)$)rectangle($(b2) +(.25,-.3)$);
%\node at ($(b1)!.5!(b2) + (0,-.75)$) {$c_0^0$};
%\draw[dashed,rounded corners=10]($(g1) + (-.25,.3)$)rectangle($(g2) +(.25,-.3)$);
%\node at ($(g1)!.5!(g2) + (0,-.75)$) {$c_1^0$};
%\draw[dashed,rounded corners=10]($(e1) + (-.25,.3)$)rectangle($(e2) +(.25,-.3)$);
%\node at ($(e1)!.5!(e2) + (0,-.75)$) {$c_0^1$};
%\draw[dashed,rounded corners=10]($(f1) + (-.25,.3)$)rectangle($(f2) +(.25,-.3)$);
%\node at ($(f1)!.5!(f2) + (0,-.75)$) {$c_1^1$};
\end{tikzpicture}
\caption{Set-BezEA linkage structure ($b = q = \ell = 2$)}
\end{figure}

==> sections/set-bezea.tex <==
\section{Set Bézier Evolutionary Algorithm}
As MM-BezEA is a niching method that divides its attention over all of the niches found by HVC, it is intractable to use MM-BezEA in highly multi-modal landscapes.
In order to overcome this limitation, a second algorithm is introduced that uses MO-RV-GOMEA \cite{mo-rv-gomea} with an adapted fitness function definition and encoding.
Rather than encoding each solution to be one Bézier curve, and clustering the population to find different niches, this algorithm, named Set-BezEA, encodes and searches for a set of $b$ Bézier curves. % uses an encoding where each solution consists of the parameters of $b$ Bezier curves.
It does so without further niching the population, which prevents this approach from falling apart in highly multi-modal landscapes.

%To enable the use of the entire population for the effective search of $b$ Bézier solutions, a new parameterization is employed.
In the original BezEA, solutions represent Bézier curves consisting of the $q$ control points $C_q$. %, which are regular solutions. %that have their parameters concatenated to a Bézier solution.
Given a problem dimensionality $\ell$, a Bézier solution thus consists of $q \cdot \ell$ parameters.
In Set-BezEA, a solution represents $b$ Bézier curves consisting of $b \cdot q$ control points $C_q$ concatenated into a set of control points denoted as $C_{q,b}$.
The control points for the $i$-th Bézier solution are denoted as $C_q^i$.
%The resulting solution set $S_{p,q,b} ( C_{q,b} )$ is then parameterized by concatenating the decision variables in the set $C_{q,b}$ as a solution.
Hence, solutions in Set-BezEA take the form $[C_q^1,  ..., C_q^b] \in \mathbb{R}^{b \cdot q \cdot \ell}$. % of $b \cdot q \cdot \ell$ parameters, also denoted as $\phi \in \mathbb{R}^{b \cdot q \cdot \ell}$.
The notation $S_{p,q}^i$, equal to the definition of $S_{p,q}$ in Equation \ref{eq:sol_set}, is used to denote the $i$-th Bézier solution of the set $S_{p,q,b}$ with $b$ Bézier solutions.

\subsection{Fitness function formulation}
In order to evaluate the newly formulated solutions, a new fitness function is proposed that can be seen in mathematical form in Equation \ref{eq:bez_fitness}.
The original fitness function formulation from BezEA is used in order to determine the constraint $L(S_{p,q,b} (\phi))$ and $\text{ HV}_{f, S_{p,q,b} (\phi)}$ values for all of the $b$ Bézier solutions combined.
%Fitness sharing \cite{fitness_sharing} is incorporated by the inclusion of the newly proposed Bézier Hill-Valley Test, whereby solution share their fitness (Hypervolume) values if the Bézier Hill-Valley test designates them to be in the same niche.
Fitness sharing \cite{fitness_sharing} is incorporated with a niching radius based on the expected edge length \cite{hillvallea}, which is checked between each of the $b$ Bézier solutions $S_{p,q}^i$.

However, fitness sharing only describes a minimal separation criterion.
Typically, in practice, decision makers would like to be able to find Bézier solutions that are diverse, yet all of high quality, while limited in number.
For this reason, the problem is defined as an MO formulation.
Herein, the second objective is a distance objective $\Delta_{S_{p,q,b}}$ that is to be maximized. 
It calculates the sum of cosine distances between all pairs of the $b$ Bézier solutions to move them apart in decision space and promote finding diverse approximation sets.

\begin{figure}
    \begin{equation}
    \small
    \label{eq:bez_fitness}
    \begin{alignedat}{3}
    &\text{maximize $f_0$: } && \text{HV}_{f, S_{p,q,b} (\phi)} && = \sum_{i=0}^{b-1} \dfrac{\text{HV}_f \left ( A^{nb} \left( S_{p,q}^i (\phi) \right) \right)}{n_i}\\
    &\text{maximize $f_1$: } && \Delta_{S_{p,q,b} (\phi)} && = \sum_{i=0}^{b-1} \sum_{j=i+1}^{b-1} \dfrac{S_{p,q}^i (\phi) \cdot S_{p,q}^j (\phi)}{||S_{p,q}^i (\phi)|| \hspace{2pt} ||S_{p,q}^j (\phi)||}\\
    &\text{with constraint: } && L\left(S_{p,q,b} (\phi) \right) && = \sum_{i=0}^{b-1}  L_b \left( S_{p,q}^i (\phi), o_{nb}^i (\phi) \right) \\
    \end{alignedat}
    \end{equation}
    \begin{equation*}
        \small
        \begin{split}
        \text{where } & f : \mathbb{R}^\ell \rightarrow \mathbb{R}^m, \phi \in \mathbb{R}^{b * q * \ell}, \\ 
         %& S_{p,q,b} : \mathbb{R}^{b \cdot q \cdot \ell} \rightarrow \left\{ \wp_0 \left( \mathcal{X} \right), ..., \wp_b \left( \mathcal{X} \right) \right\}, \\ 
         %& S_{p,q,b} : \mathbb{R}^{b \cdot q \cdot \ell} \rightarrow \left\{ S_{p,q}^1(\phi), ..., S_{p,q}^b(\phi) \right\}, \\ 
         & A^{nb} : \text{solution set }S_{p,q}^i(\phi) \rightarrow \text{approximation set } \mathcal{A}_{p,q,o_{nb}}^i \\
         & n_i \text{ number of Bézier curves in same niche as } S_{p,q}^i \\ 
         & o_{nb}^i (\phi)\text{ the navigational order of the }i\text{-th Bézier solution} \\
         & L_b(S_{p,q}^i (\phi), o_{nb}^i (\phi)) \text{ the Bézier constraint function} \\
        \end{split}
    \end{equation*}
\end{figure}

\subsection{Adaptive steering}
The MO formulation of the previous section creates a trade-off between finding far apart solutions at the edges of the search space and those closer to the PSs.
However, especially assuming the global optimum cannot be obtained, the primary goal is to obtain distinct solutions that are of high quality.
%In (M)MOPs the size and shape of the PF varies largely depending on the problem.
Most (M)MOEAs try to find improvements spread over the entire PF, whereas in some situation only a part of the PF is interesting.
In order to steer Set-BezEA towards the interesting parts of the PF, the notion of adaptive steering \cite{adaptive_steering} can be used on the first objective value.
%Therefore, adaptive steering \cite{adaptive_steering} is implemented for the first objective value.
Starting at allowing Bézier set solutions to be within $50\%$ of the best achieved cumulative HV it scales linearly in 50 generations to $99\%$.
This will force all solutions towards higher HV values when combined with constraint domination \cite{constraint_dom}.

\subsection{Linkage structure and partial evaluations}
To optimize for the new fitness formulation, Set-BezEA uses MO-RV-GOMEA, which uses a linkage model \cite{ltm} to determine which variables are to be changed at the same time.
It is often taken to be a linkage tree that is constructed using the unweighted pair group method with arithmetic mean (UPGMA) \cite{upgma} to iteratively cluster decision variables.
A new linkage structure is designed for Set-BezEA to guide MO-RV-GOMEA and allow it to exploit the underlying structure of a problem.
For this new linkage structure, the ideas behind the linkage structures defined for BezEA and UHV-GOMEA were combined \cite{bezea}.

When the $j$-th decision variable of a control point in Bézier curve changes, the $j$-th decision variable of all test solutions of the approximation set $S_{p,q}^i(C_q)$ changes, which makes it beneficial to change the same decision variable for all $q$ control points of a Bézier curve at once.
This is the first layer of the new linkage structure, where, for each of the $b$ Bézier solutions, their $j$-th decision variables of all $q$ control points are grouped.
Subsequently, the $\ell$ clusters of $q$ decision variables for one Bézier solution are hierarchically grouped using UPGMA. % until all decision variables of one Bézier solution are clustered.
The second layer combines the $b$ resulting groups of the decision variables of all $b$ Bézier solutions by concatenating them into one large linkage tree. 

%\input{sections/set-bezea-linkage-tree}

The newly defined linkage structure enables MO-RV-GOMEA to perform partial evaluations in all situations.
Even if the underlying problem setting is black-box in nature, partial evaluations are enabled by the second layer, as each of these Bézier curves can be evaluated separately for its HV contribution to the first objective.
%Even if the underlying problem setting is black-box in nature, thus preventing the use of the first layer that combines decision variables of control points of one Bézier cure, partial evaluations are still possible as each of the $b$ Bézier solutions can be evaluated separately.
%This is enabled by the second layer that concatenates each of the $b$ Bézier solutions, as each of these curves can be evaluated separately for its hypervolume contribution to the first objective.
The second distance objective always has to be recalculated, but it does not require any evaluations of the original fitness function.

\subsection{MO-RV-GOMEA adaptations}
%The approximation sets $S_{p,q}^i(C_q)$ are defined by their control points $C_q^i$, of which the control points $\boldsymbol{c}_1^i$ and $\boldsymbol{c}_{q}^i$ are the extremes.
The approximation sets $S_{p,q}^i(C_q)$, defined by the Bézier curves, are evaluated with the HV indicator that makes use of a reference point.
But, the choice of reference point highly influences whether or not the extremes of the PF can be found \cite{ref_point}.

The control points $\boldsymbol{c}_1^i$ and $\boldsymbol{c}_{q}^i$ are likely to come as close as possible to the constraint region, defined by being dominated by the reference point, to maximize the HV.
However, if one of these two control points falls just slightly in the constraint region, the constraint function $C(S_{p,q,b} (\phi))$ combined with constraint domination will make it one of the worst performing solutions.
Furthermore, MO-RV-GOMEA makes use of the Gene-pool Optimal Mixing (GOM) variation operator, thereby disallowing deterioration of fitness.
These two effects combined, quickly reduce the variance in the population, since very slight adjustments can significantly deteriorate the individual.
In order to overcome this downside, the GOM part of MO-RV-GOMEA has been adapted to allow deterioration of the objective values, i.e., accepting a modification that would otherwise have been rejected, with a probability of $5\%$, as was previously done in RV-GOMEA \cite{rv_gomea}.
This adaptation enables MO-RV-GOMEA to effectively search the outer regions of the search space close to the constraint space by preserving more variance.

==> sections/tables-per-indicator-other-test-points.tex <==
\subsubsection{p = 10}
\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA                 & MO-Ring-PSO-SCD               & MO-RV-GOMEA                   & Sets-BezEA                    \\
\hline
 MinDist   & 1.18e+02 (±6.26e-08)          & 1.18e+02 (±4.51e-03)          & \textbf{1.19e+02 (±1.66e-02)} & 1.18e+02 (±1.01e-03)          & 1.18e+02 (±3.48e-04)          \\
 MMF12     & 1.77e+00 (±3.13e-02)          & \textbf{2.07e+00 (±6.49e-04)} & 2.05e+00 (±1.27e-03)          & 2.07e+00 (±1.66e-04)          & 1.72e+00 (±1.62e-01)          \\
 MMF14     & 5.70e+00 (±1.05e-08)          & \textbf{5.71e+00 (±2.92e-04)} & 5.53e+00 (±1.14e-01)          & 5.71e+00 (±5.08e-05)          & 5.70e+00 (±2.24e-13)          \\
 MMF15     & 5.63e+00 (±2.42e-08)          & \textbf{5.64e+00 (±1.36e-04)} & 5.39e+00 (±8.63e-02)          & 5.64e+00 (±5.93e-05)          & 5.63e+00 (±2.14e-11)          \\
 OmniTest  & \textbf{9.55e-01 (±4.14e-10)} & 9.52e-01 (±2.77e-04)          & 9.29e-01 (±3.46e-04)          & 9.51e-01 (±1.01e-04)          & \textbf{9.55e-01 (±4.61e-05)} \\
 SSUF1     & 5.99e-01 (±8.08e-03)          & \textbf{8.23e-01 (±2.33e-04)} & 8.02e-01 (±4.04e-04)          & \textbf{8.23e-01 (±1.45e-04)} & 6.40e-01 (±4.10e-02)          \\
 SSUF3     & 6.38e-01 (±1.32e-09)          & \textbf{8.23e-01 (±7.24e-04)} & 8.00e-01 (±2.17e-03)          & \textbf{8.23e-01 (±3.32e-04)} & 6.30e-01 (±5.09e-02)          \\
 SymPart1  & \textbf{1.18e+02 (±3.40e-08)} & 1.18e+02 (±7.74e-03)          & 1.17e+02 (±8.45e-03)          & 1.18e+02 (±9.74e-04)          & 1.15e+02 (±2.27e+00)          \\
 SymPart2  & \textbf{1.18e+02 (±2.83e-08)} & 1.18e+02 (±7.66e-03)          & 1.17e+02 (±1.34e-02)          & 1.18e+02 (±1.58e-03)          & \textbf{1.17e+02 (±1.42e+00)} \\
 SymPart3  & \textbf{1.18e+02 (±2.56e-07)} & 1.18e+02 (±8.56e-03)          & 1.17e+02 (±1.65e-02)          & 1.18e+02 (±1.95e-03)          & 1.18e+02 (±1.03e-01)          \\
 TwoOnOne  & 1.13e+02 (±9.03e-08)          & 1.13e+02 (±5.50e-05)          & \textbf{1.35e+02 (±1.39e-04)} & 1.13e+02 (±5.29e-05)          & 1.13e+02 (±6.48e-03)          \\
\hline
\end{tabular}
\caption{Results for HV indicator}
\label{tab:res_hv}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA                 & MO-Ring-PSO-SCD               & MO-RV-GOMEA          & Sets-BezEA                    \\
\hline
 MinDist   & \textbf{9.27e-04 (±2.92e-06)} & 2.08e-02 (±1.12e-03)          & 1.44e-02 (±1.31e-03)          & 1.33e+00 (±8.55e-01) & 2.10e-03 (±2.15e-03)          \\
 MMF12     & 6.12e-02 (±1.04e-02)          & 5.13e-02 (±1.15e-03)          & \textbf{4.35e-02 (±2.52e-04)} & 7.42e-02 (±3.51e-05) & 2.25e-01 (±3.55e-02)          \\
 MMF14     & 2.51e-04 (±8.27e-07)          & 2.71e-03 (±7.00e-05)          & 4.29e-03 (±4.18e-04)          & 2.27e-01 (±7.86e-02) & \textbf{2.50e-04 (±1.96e-10)} \\
 MMF15     & \textbf{3.50e-03 (±7.10e-06)} & 3.78e-03 (±7.92e-05)          & 4.09e-03 (±8.89e-05)          & 3.17e-02 (±4.07e-05) & \textbf{3.50e-03 (±1.41e-07)} \\
 OmniTest  & 8.93e-02 (±1.25e-01)          & 1.77e-02 (±1.26e-03)          & \textbf{1.49e-02 (±1.52e-03)} & 1.42e+00 (±4.09e-01) & 1.68e+00 (±2.05e-01)          \\
 SSUF1     & 1.51e-01 (±5.82e-02)          & 3.19e-02 (±8.63e-04)          & \textbf{2.66e-02 (±5.50e-03)} & 3.47e-01 (±2.52e-02) & 3.88e-01 (±1.07e-01)          \\
 SSUF3     & 2.97e-01 (±1.21e-01)          & \textbf{1.02e-02 (±7.03e-04)} & 1.94e-02 (±3.13e-03)          & 2.05e-01 (±8.98e-02) & 4.07e-01 (±1.28e-01)          \\
 SymPart1  & 1.08e-01 (±2.85e-01)          & \textbf{2.78e-02 (±5.70e-04)} & 3.89e-02 (±6.22e-03)          & 7.71e+00 (±2.15e+00) & 9.22e+00 (±8.62e-01)          \\
 SymPart2  & 2.06e-01 (±3.96e-01)          & \textbf{2.83e-02 (±3.15e-03)} & 4.31e-02 (±4.04e-03)          & 6.41e+00 (±1.51e+00) & 8.57e+00 (±6.53e-01)          \\
 SymPart3  & 9.64e-01 (±8.60e-01)          & \textbf{9.81e-02 (±2.16e-01)} & \textbf{3.99e-02 (±1.43e-02)} & 6.46e+00 (±2.41e+00) & 7.85e+00 (±1.35e+00)          \\
 TwoOnOne  & 5.18e-03 (±4.83e-03)          & 2.21e-02 (±2.46e-04)          & 4.15e-02 (±2.00e-02)          & 1.97e-01 (±3.01e-02) & \textbf{5.59e-02 (±1.58e-01)} \\
\hline
\end{tabular}
\caption{Results for IGDX indicator}
\label{tab:res_igdx}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA                 & MO-Ring-PSO-SCD               & MO-RV-GOMEA          & Sets-BezEA                    \\
\hline
 MinDist   & \textbf{1.06e+03 (±1.90e+01)} & 4.81e+01 (±2.56e+00)          & 6.96e+01 (±6.46e+00)          & 1.49e+00 (±1.96e+00) & 7.38e+02 (±3.30e+02)          \\
 MMF12     & 9.59e+00 (±4.76e+00)          & 1.00e+01 (±2.22e-01)          & \textbf{1.53e+01 (±9.53e-02)} & 6.89e+00 (±4.43e-03) & 3.26e-01 (±6.34e-01)          \\
 MMF14     & 3.98e+03 (±1.31e+01)          & 3.69e+02 (±9.31e+00)          & 2.35e+02 (±2.21e+01)          & 2.87e+00 (±5.73e+00) & \textbf{4.00e+03 (±3.17e-03)} \\
 MMF15     & \textbf{2.86e+02 (±5.79e-01)} & 2.65e+02 (±5.55e+00)          & 2.44e+02 (±5.35e+00)          & 3.15e+01 (±4.05e-02) & \textbf{2.86e+02 (±1.15e-02)} \\
 OmniTest  & 5.09e+01 (±4.04e+01)          & 5.66e+01 (±3.50e+00)          & \textbf{6.71e+01 (±7.39e+00)} & 2.37e-01 (±3.82e-01) & 2.11e-02 (±4.60e-02)          \\
 SSUF1     & 5.52e+00 (±2.03e+00)          & 3.14e+01 (±8.59e-01)          & \textbf{3.84e+01 (±6.49e+00)} & 1.87e+00 (±6.41e-01) & 3.36e-01 (±2.74e-01)          \\
 SSUF3     & 1.72e+00 (±2.25e+00)          & \textbf{9.85e+01 (±6.61e+00)} & 4.59e+01 (±8.43e+00)          & 3.64e+00 (±2.07e+00) & 1.35e-01 (±1.16e-01)          \\
 SymPart1  & \textbf{7.02e+02 (±5.33e+02)} & 3.60e+01 (±7.32e-01)          & 2.62e+01 (±3.84e+00)          & 6.82e-03 (±2.05e-02) & 8.45e-04 (±2.29e-03)          \\
 SymPart2  & \textbf{7.89e+02 (±5.15e+02)} & 3.56e+01 (±3.12e+00)          & 2.31e+01 (±2.22e+00)          & 1.55e-02 (±2.02e-02) & 5.01e-04 (±3.69e-04)          \\
 SymPart3  & 2.03e+01 (±5.63e+01)          & \textbf{3.83e+01 (±1.54e+01)} & \textbf{2.70e+01 (±7.37e+00)} & 1.43e-02 (±2.23e-02) & 1.11e-03 (±7.09e-04)          \\
 TwoOnOne  & 2.57e+02 (±7.08e+01)          & 4.51e+01 (±4.77e-01)          & 2.29e+01 (±1.33e+01)          & 3.48e+00 (±1.24e+00) & \textbf{2.72e+02 (±9.70e+01)} \\
\hline
\end{tabular}
\caption{Results for PSP indicator}
\label{tab:res_psp}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA        & MO-Ring-PSO-SCD      & MO-RV-GOMEA                   & Sets-BezEA                    \\
\hline
 MinDist   & \textbf{1.00e+00 (±0.00e+00)} & 5.98e-01 (±2.12e-02) & 7.65e-01 (±4.66e-03) & 9.24e-01 (±1.01e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MMF12     & \textbf{1.00e+00 (±0.00e+00)} & 5.95e-01 (±1.75e-02) & 6.34e-01 (±1.12e-02) & \textbf{1.00e+00 (±0.00e+00)} & \textbf{1.00e+00 (±0.00e+00)} \\
 MMF14     & \textbf{1.00e+00 (±0.00e+00)} & 5.84e-01 (±2.48e-02) & 8.68e-01 (±1.14e-02) & 9.27e-01 (±1.47e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MMF15     & \textbf{1.00e+00 (±0.00e+00)} & 5.88e-01 (±3.02e-02) & 8.62e-01 (±8.55e-03) & \textbf{1.00e+00 (±0.00e+00)} & \textbf{1.00e+00 (±0.00e+00)} \\
 OmniTest  & \textbf{1.00e+00 (±0.00e+00)} & 5.62e-01 (±2.04e-02) & 7.27e-01 (±1.02e-02) & 7.53e-01 (±1.81e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SSUF1     & \textbf{1.00e+00 (±0.00e+00)} & 5.35e-01 (±1.09e-02) & 7.85e-01 (±5.97e-03) & 5.56e-01 (±4.25e-02)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SSUF3     & \textbf{1.00e+00 (±0.00e+00)} & 6.82e-01 (±3.37e-02) & 5.00e-01 (±7.07e-03) & 8.87e-01 (±1.23e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SymPart1  & \textbf{1.00e+00 (±0.00e+00)} & 5.82e-01 (±3.76e-02) & 6.87e-01 (±1.03e-02) & 7.14e-01 (±1.66e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SymPart2  & \textbf{1.00e+00 (±0.00e+00)} & 5.79e-01 (±2.65e-02) & 5.68e-01 (±1.28e-02) & 7.60e-01 (±1.15e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SymPart3  & \textbf{1.00e+00 (±0.00e+00)} & 6.07e-01 (±3.61e-02) & 5.33e-01 (±1.34e-02) & 8.49e-01 (±1.53e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 TwoOnOne  & \textbf{1.00e+00 (±0.00e+00)} & 5.95e-01 (±2.90e-02) & 7.44e-01 (±9.55e-03) & 8.34e-01 (±1.14e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
\hline
\end{tabular}
\caption{Results for Smoothness indicator}
\label{tab:res_smooth}
\end{table*}

\clearpage
\subsubsection{p = 9}
\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA             & MO-HillVallEA                 & MO-Ring-PSO-SCD               & MO-RV-GOMEA          & Sets-BezEA           \\
\hline
 MinDist   & 1.18e+02 (±1.03e-07) & 1.18e+02 (±4.51e-03)          & \textbf{1.19e+02 (±1.66e-02)} & 1.17e+02 (±1.44e-03) & 1.18e+02 (±4.51e-08) \\
 MMF12     & 1.78e+00 (±8.99e-07) & \textbf{2.07e+00 (±6.49e-04)} & 2.05e+00 (±1.27e-03)          & 2.06e+00 (±1.59e-04) & 1.80e+00 (±1.51e-01) \\
 MMF14     & 5.68e+00 (±1.38e-08) & \textbf{5.71e+00 (±2.92e-04)} & 5.53e+00 (±1.14e-01)          & 5.70e+00 (±1.72e-05) & 5.68e+00 (±4.82e-15) \\
 MMF15     & 5.61e+00 (±2.38e-02) & \textbf{5.64e+00 (±1.36e-04)} & 5.39e+00 (±8.63e-02)          & 5.63e+00 (±1.03e-05) & 5.61e+00 (±6.33e-12) \\
 OmniTest  & 9.51e-01 (±2.48e-10) & \textbf{9.52e-01 (±2.77e-04)} & 9.29e-01 (±3.46e-04)          & 9.47e-01 (±7.27e-05) & 9.18e-01 (±9.71e-02) \\
 SSUF1     & 6.03e-01 (±2.84e-06) & \textbf{8.23e-01 (±2.33e-04)} & 8.02e-01 (±4.04e-04)          & 8.17e-01 (±1.42e-04) & 6.27e-01 (±3.90e-02) \\
 SSUF3     & 6.30e-01 (±2.24e-02) & \textbf{8.23e-01 (±7.24e-04)} & 8.00e-01 (±2.17e-03)          & 8.17e-01 (±2.51e-04) & 5.91e-01 (±5.59e-02) \\
 SymPart1  & 1.18e+02 (±4.45e-08) & \textbf{1.18e+02 (±7.74e-03)} & 1.17e+02 (±8.45e-03)          & 1.17e+02 (±9.07e-04) & 1.16e+02 (±1.87e+00) \\
 SymPart2  & 1.18e+02 (±2.84e-08) & \textbf{1.18e+02 (±7.66e-03)} & 1.17e+02 (±1.34e-02)          & 1.17e+02 (±3.61e-03) & 1.15e+02 (±1.64e+00) \\
 SymPart3  & 1.18e+02 (±1.23e-07) & \textbf{1.18e+02 (±8.56e-03)} & 1.17e+02 (±1.65e-02)          & 1.17e+02 (±3.21e-03) & 1.16e+02 (±1.86e+00) \\
 TwoOnOne  & 1.13e+02 (±5.10e-08) & 1.13e+02 (±5.50e-05)          & \textbf{1.35e+02 (±1.39e-04)} & 1.13e+02 (±1.11e-04) & 1.13e+02 (±7.04e-02) \\
\hline
\end{tabular}
\caption{Results for HV indicator}
\label{tab:res_hv}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA                 & MO-Ring-PSO-SCD               & MO-RV-GOMEA          & Sets-BezEA                    \\
\hline
 MinDist   & 1.08e-03 (±9.26e-06)          & 2.08e-02 (±1.12e-03)          & 1.44e-02 (±1.31e-03)          & 1.34e+00 (±8.54e-01) & \textbf{1.07e-03 (±1.16e-09)} \\
 MMF12     & 5.75e-02 (±1.17e-02)          & 5.13e-02 (±1.15e-03)          & \textbf{4.35e-02 (±2.52e-04)} & 7.52e-02 (±4.28e-04) & 2.00e-01 (±5.71e-02)          \\
 MMF14     & 4.94e-04 (±7.32e-04)          & 2.71e-03 (±7.00e-05)          & 4.29e-03 (±4.18e-04)          & 2.35e-01 (±6.83e-02) & \textbf{2.50e-04 (±4.71e-12)} \\
 MMF15     & \textbf{4.00e-03 (±1.50e-03)} & 3.78e-03 (±7.92e-05)          & 4.09e-03 (±8.89e-05)          & 3.66e-02 (±5.69e-05) & \textbf{3.50e-03 (±1.11e-07)} \\
 OmniTest  & 3.21e-02 (±5.68e-02)          & 1.77e-02 (±1.26e-03)          & \textbf{1.49e-02 (±1.52e-03)} & 1.46e+00 (±4.36e-01) & 1.71e+00 (±2.00e-01)          \\
 SSUF1     & 1.67e-01 (±4.62e-02)          & 3.19e-02 (±8.63e-04)          & \textbf{2.66e-02 (±5.50e-03)} & 3.62e-01 (±2.65e-02) & 3.94e-01 (±8.22e-02)          \\
 SSUF3     & 2.07e-01 (±1.22e-01)          & \textbf{1.02e-02 (±7.03e-04)} & 1.94e-02 (±3.13e-03)          & 2.15e-01 (±8.87e-02) & 4.97e-01 (±1.30e-01)          \\
 SymPart1  & 1.54e-02 (±3.25e-02)          & \textbf{2.78e-02 (±5.70e-04)} & 3.89e-02 (±6.22e-03)          & 7.72e+00 (±2.15e+00) & 9.15e+00 (±8.60e-01)          \\
 SymPart2  & \textbf{2.32e-03 (±3.84e-03)} & 2.83e-02 (±3.15e-03)          & 4.31e-02 (±4.04e-03)          & 6.70e+00 (±1.45e+00) & 9.84e+00 (±4.76e-01)          \\
 SymPart3  & 5.41e-01 (±5.63e-01)          & \textbf{9.81e-02 (±2.16e-01)} & \textbf{3.99e-02 (±1.43e-02)} & 6.47e+00 (±2.40e+00) & 9.02e+00 (±1.33e+00)          \\
 TwoOnOne  & \textbf{3.51e-03 (±7.92e-05)} & 2.21e-02 (±2.46e-04)          & 4.15e-02 (±2.00e-02)          & 2.12e-01 (±3.18e-02) & 2.05e-01 (±3.07e-01)          \\
\hline
\end{tabular}
\caption{Results for IGDX indicator}
\label{tab:res_igdx}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA                 & MO-Ring-PSO-SCD               & MO-RV-GOMEA          & Sets-BezEA                    \\
\hline
 MinDist   & \textbf{9.06e+02 (±1.57e+01)} & 4.81e+01 (±2.56e+00)          & 6.96e+01 (±6.46e+00)          & 1.45e+00 (±1.90e+00) & 8.69e+02 (±8.45e-04)          \\
 MMF12     & 1.08e+01 (±5.98e+00)          & 1.00e+01 (±2.22e-01)          & \textbf{1.53e+01 (±9.53e-02)} & 6.80e+00 (±3.96e-02) & 5.80e-01 (±9.98e-01)          \\
 MMF14     & 3.63e+03 (±1.09e+03)          & 3.69e+02 (±9.31e+00)          & 2.35e+02 (±2.21e+01)          & 2.04e+00 (±4.07e+00) & \textbf{4.00e+03 (±7.89e-05)} \\
 MMF15     & \textbf{2.69e+02 (±5.03e+01)} & 2.65e+02 (±5.55e+00)          & 2.44e+02 (±5.35e+00)          & 2.73e+01 (±4.24e-02) & \textbf{2.86e+02 (±9.04e-03)} \\
 OmniTest  & 6.72e+01 (±2.73e+01)          & 5.66e+01 (±3.50e+00)          & \textbf{6.71e+01 (±7.39e+00)} & 2.34e-01 (±3.78e-01) & 5.14e-03 (±1.18e-02)          \\
 SSUF1     & 4.51e+00 (±2.49e+00)          & 3.14e+01 (±8.59e-01)          & \textbf{3.84e+01 (±6.49e+00)} & 1.44e+00 (±4.67e-01) & 2.43e-01 (±1.67e-01)          \\
 SSUF3     & 2.89e+00 (±2.45e+00)          & \textbf{9.85e+01 (±6.61e+00)} & 4.59e+01 (±8.43e+00)          & 3.01e+00 (±1.66e+00) & 1.91e-02 (±2.77e-02)          \\
 SymPart1  & \textbf{7.65e+02 (±3.78e+02)} & 3.60e+01 (±7.32e-01)          & 2.62e+01 (±3.84e+00)          & 6.79e-03 (±2.04e-02) & 9.26e-04 (±2.53e-03)          \\
 SymPart2  & \textbf{8.73e+02 (±2.73e+02)} & 3.56e+01 (±3.12e+00)          & 2.31e+01 (±2.22e+00)          & 1.42e-02 (±1.90e-02) & 7.99e-05 (±2.35e-04)          \\
 SymPart3  & 5.78e+00 (±7.28e+00)          & \textbf{3.83e+01 (±1.54e+01)} & \textbf{2.70e+01 (±7.37e+00)} & 1.42e-02 (±2.22e-02) & 1.62e-03 (±2.47e-03)          \\
 TwoOnOne  & \textbf{2.84e+02 (±6.35e+00)} & 4.51e+01 (±4.77e-01)          & 2.29e+01 (±1.33e+01)          & 3.02e+00 (±1.30e+00) & \textbf{1.99e+02 (±1.30e+02)} \\
\hline
\end{tabular}
\caption{Results for PSP indicator}
\label{tab:res_psp}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA        & MO-Ring-PSO-SCD      & MO-RV-GOMEA                   & Sets-BezEA                    \\
\hline
 MinDist   & \textbf{1.00e+00 (±0.00e+00)} & 5.98e-01 (±2.12e-02) & 7.65e-01 (±4.66e-03) & 9.01e-01 (±1.40e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MMF12     & \textbf{1.00e+00 (±0.00e+00)} & 5.95e-01 (±1.75e-02) & 6.34e-01 (±1.12e-02) & \textbf{1.00e+00 (±0.00e+00)} & \textbf{1.00e+00 (±0.00e+00)} \\
 MMF14     & \textbf{1.00e+00 (±0.00e+00)} & 5.84e-01 (±2.48e-02) & 8.68e-01 (±1.14e-02) & 9.43e-01 (±1.15e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MMF15     & \textbf{1.00e+00 (±0.00e+00)} & 5.88e-01 (±3.02e-02) & 8.62e-01 (±8.55e-03) & \textbf{1.00e+00 (±0.00e+00)} & \textbf{1.00e+00 (±0.00e+00)} \\
 OmniTest  & \textbf{1.00e+00 (±0.00e+00)} & 5.62e-01 (±2.04e-02) & 7.27e-01 (±1.02e-02) & 7.68e-01 (±1.87e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SSUF1     & \textbf{1.00e+00 (±0.00e+00)} & 5.35e-01 (±1.09e-02) & 7.85e-01 (±5.97e-03) & 5.42e-01 (±4.75e-02)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SSUF3     & \textbf{1.00e+00 (±0.00e+00)} & 6.82e-01 (±3.37e-02) & 5.00e-01 (±7.07e-03) & 8.86e-01 (±1.10e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SymPart1  & \textbf{1.00e+00 (±0.00e+00)} & 5.82e-01 (±3.76e-02) & 6.87e-01 (±1.03e-02) & 6.96e-01 (±2.17e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SymPart2  & \textbf{1.00e+00 (±0.00e+00)} & 5.79e-01 (±2.65e-02) & 5.68e-01 (±1.28e-02) & 8.21e-01 (±7.38e-02)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SymPart3  & \textbf{1.00e+00 (±0.00e+00)} & 6.07e-01 (±3.61e-02) & 5.33e-01 (±1.34e-02) & 8.66e-01 (±1.31e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 TwoOnOne  & \textbf{1.00e+00 (±0.00e+00)} & 5.95e-01 (±2.90e-02) & 7.44e-01 (±9.55e-03) & 7.99e-01 (±1.60e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
\hline
\end{tabular}
\caption{Results for Smoothness indicator}
\label{tab:res_smooth}
\end{table*}

\clearpage
\subsubsection{p = 8}
\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA                 & MO-Ring-PSO-SCD               & MO-RV-GOMEA                   & Sets-BezEA                    \\
\hline
 MinDist   & 1.17e+02 (±7.63e-08)          & 1.17e+02 (±1.37e-02)          & \textbf{1.19e+02 (±1.66e-02)} & 1.17e+02 (±8.69e-04)          & 1.17e+02 (±4.43e-09)          \\
 MMF12     & 1.78e+00 (±6.83e-07)          & \textbf{2.06e+00 (±2.70e-03)} & 2.05e+00 (±1.27e-03)          & \textbf{2.06e+00 (±1.52e-04)} & 1.72e+00 (±1.51e-01)          \\
 MMF14     & 5.66e+00 (±1.09e-08)          & \textbf{5.67e+00 (±4.70e-04)} & 5.53e+00 (±1.14e-01)          & 5.67e+00 (±1.67e-04)          & 5.66e+00 (±2.10e-15)          \\
 MMF15     & 5.59e+00 (±1.33e-02)          & \textbf{5.60e+00 (±2.66e-04)} & 5.39e+00 (±8.63e-02)          & 5.60e+00 (±8.02e-05)          & 5.59e+00 (±8.28e-15)          \\
 OmniTest  & 9.45e-01 (±1.91e-10)          & 9.42e-01 (±1.35e-04)          & 9.29e-01 (±3.46e-04)          & 9.42e-01 (±6.21e-05)          & \textbf{9.45e-01 (±3.03e-05)} \\
 SSUF1     & 5.92e-01 (±1.71e-02)          & \textbf{8.11e-01 (±2.89e-04)} & 8.02e-01 (±4.04e-04)          & \textbf{8.11e-01 (±1.04e-04)} & 6.22e-01 (±3.51e-02)          \\
 SSUF3     & 6.29e-01 (±2.00e-02)          & \textbf{8.11e-01 (±6.26e-04)} & 8.00e-01 (±2.17e-03)          & \textbf{8.11e-01 (±1.71e-04)} & 5.91e-01 (±5.21e-02)          \\
 SymPart1  & \textbf{1.17e+02 (±2.59e-08)} & 1.17e+02 (±1.14e-02)          & 1.17e+02 (±8.45e-03)          & 1.17e+02 (±1.05e-03)          & 1.16e+02 (±2.16e+00)          \\
 SymPart2  & \textbf{1.17e+02 (±1.90e-08)} & 1.17e+02 (±6.09e-03)          & 1.17e+02 (±1.34e-02)          & 1.17e+02 (±5.06e-03)          & 1.16e+02 (±2.08e+00)          \\
 SymPart3  & \textbf{1.17e+02 (±4.69e-06)} & 1.17e+02 (±1.26e-02)          & 1.17e+02 (±1.65e-02)          & 1.17e+02 (±3.73e-03)          & 1.17e+02 (±6.36e-01)          \\
 TwoOnOne  & 1.13e+02 (±7.98e-08)          & 1.13e+02 (±2.06e-04)          & \textbf{1.35e+02 (±1.39e-04)} & 1.13e+02 (±1.15e-04)          & 1.13e+02 (±4.84e-02)          \\
\hline
\end{tabular}
\caption{Results for HV indicator}
\label{tab:res_hv}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA                 & MO-Ring-PSO-SCD               & MO-RV-GOMEA          & Sets-BezEA                    \\
\hline
 MinDist   & 1.33e-03 (±1.92e-06)          & 2.04e-02 (±1.23e-03)          & 1.44e-02 (±1.31e-03)          & 1.54e+00 (±7.64e-01) & \textbf{1.32e-03 (±1.79e-09)} \\
 MMF12     & 4.82e-02 (±1.24e-02)          & 5.13e-02 (±1.24e-03)          & \textbf{4.35e-02 (±2.52e-04)} & 7.55e-02 (±3.23e-05) & 2.36e-01 (±8.71e-03)          \\
 MMF14     & 1.31e-03 (±3.18e-03)          & 2.70e-03 (±8.00e-05)          & 4.29e-03 (±4.18e-04)          & 2.43e-01 (±5.84e-02) & \textbf{2.50e-04 (±5.34e-13)} \\
 MMF15     & 5.02e-03 (±3.05e-03)          & 3.78e-03 (±3.74e-05)          & 4.09e-03 (±8.89e-05)          & 4.06e-02 (±4.80e-05) & \textbf{3.50e-03 (±5.33e-09)} \\
 OmniTest  & 1.37e-02 (±4.21e-03)          & \textbf{1.38e-02 (±6.83e-04)} & 1.49e-02 (±1.52e-03)          & 1.48e+00 (±4.25e-01) & 1.65e+00 (±7.51e-02)          \\
 SSUF1     & 1.77e-01 (±4.04e-02)          & 3.20e-02 (±7.16e-04)          & \textbf{2.66e-02 (±5.50e-03)} & 3.83e-01 (±2.28e-02) & 4.19e-01 (±1.14e-01)          \\
 SSUF3     & 2.07e-01 (±1.01e-01)          & \textbf{8.96e-03 (±1.42e-03)} & 1.94e-02 (±3.13e-03)          & 2.21e-01 (±9.04e-02) & 4.41e-01 (±1.24e-01)          \\
 SymPart1  & \textbf{2.52e-03 (±2.24e-03)} & 2.88e-02 (±1.45e-03)          & 3.89e-02 (±6.22e-03)          & 7.98e+00 (±2.16e+00) & 9.09e+00 (±8.20e-01)          \\
 SymPart2  & \textbf{9.24e-03 (±1.33e-02)} & 2.78e-02 (±6.47e-04)          & 4.31e-02 (±4.04e-03)          & 6.88e+00 (±1.72e+00) & 8.95e+00 (±6.95e-01)          \\
 SymPart3  & 4.17e-01 (±3.92e-01)          & \textbf{2.33e-02 (±1.28e-03)} & 3.99e-02 (±1.43e-02)          & 6.72e+00 (±2.18e+00) & 8.03e+00 (±1.34e+00)          \\
 TwoOnOne  & \textbf{3.57e-03 (±4.07e-05)} & 2.22e-02 (±4.33e-04)          & 4.15e-02 (±2.00e-02)          & 2.27e-01 (±2.86e-02) & 1.28e-01 (±2.50e-01)          \\
\hline
\end{tabular}
\caption{Results for IGDX indicator}
\label{tab:res_igdx}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA                 & MO-Ring-PSO-SCD               & MO-RV-GOMEA          & Sets-BezEA                    \\
\hline
 MinDist   & \textbf{7.42e+02 (±1.51e+01)} & 4.91e+01 (±3.04e+00)          & 6.96e+01 (±6.46e+00)          & 8.59e-01 (±1.43e+00) & 6.98e+02 (±9.94e-04)          \\
 MMF12     & 1.53e+01 (±6.74e+00)          & 1.00e+01 (±2.82e-01)          & \textbf{1.53e+01 (±9.53e-02)} & 6.78e+00 (±3.87e-03) & 1.55e-01 (±1.93e-01)          \\
 MMF14     & 3.60e+03 (±1.17e+03)          & 3.71e+02 (±1.05e+01)          & 2.35e+02 (±2.21e+01)          & 1.63e+00 (±3.35e+00) & \textbf{4.00e+03 (±1.51e-05)} \\
 MMF15     & 2.47e+02 (±7.81e+01)          & 2.64e+02 (±2.61e+00)          & 2.44e+02 (±5.35e+00)          & 2.46e+01 (±2.91e-02) & \textbf{2.86e+02 (±4.34e-04)} \\
 OmniTest  & 7.09e+01 (±1.44e+01)          & \textbf{7.28e+01 (±3.68e+00)} & 6.71e+01 (±7.39e+00)          & 2.17e-01 (±3.75e-01) & 1.88e-02 (±2.16e-02)          \\
 SSUF1     & 4.36e+00 (±1.79e+00)          & 3.12e+01 (±7.00e-01)          & \textbf{3.84e+01 (±6.49e+00)} & 1.26e+00 (±4.00e-01) & 2.38e-01 (±2.16e-01)          \\
 SSUF3     & 3.07e+00 (±2.88e+00)          & \textbf{1.14e+02 (±1.61e+01)} & 4.59e+01 (±8.43e+00)          & 2.81e+00 (±1.54e+00) & 4.23e-02 (±4.12e-02)          \\
 SymPart1  & \textbf{5.91e+02 (±2.57e+02)} & 3.49e+01 (±1.70e+00)          & 2.62e+01 (±3.84e+00)          & 5.22e-03 (±1.56e-02) & 1.70e-03 (±3.23e-03)          \\
 SymPart2  & \textbf{4.08e+02 (±3.00e+02)} & 3.60e+01 (±8.29e-01)          & 2.31e+01 (±2.22e+00)          & 1.41e-02 (±1.88e-02) & 3.30e-04 (±3.63e-04)          \\
 SymPart3  & 1.06e+01 (±1.61e+01)          & \textbf{4.30e+01 (±2.44e+00)} & 2.70e+01 (±7.37e+00)          & 1.19e-02 (±2.00e-02) & 7.27e-04 (±8.00e-04)          \\
 TwoOnOne  & \textbf{2.79e+02 (±3.19e+00)} & 4.49e+01 (±8.66e-01)          & 2.29e+01 (±1.33e+01)          & 2.77e+00 (±1.13e+00) & \textbf{2.23e+02 (±1.11e+02)} \\
\hline
\end{tabular}
\caption{Results for PSP indicator}
\label{tab:res_psp}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{llllll}
\hline
 Problem   & MM-BezEA                      & MO-HillVallEA        & MO-Ring-PSO-SCD      & MO-RV-GOMEA                   & Sets-BezEA                    \\
\hline
 MinDist   & \textbf{1.00e+00 (±0.00e+00)} & 5.95e-01 (±2.51e-02) & 7.65e-01 (±4.66e-03) & 9.32e-01 (±1.13e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MMF12     & \textbf{1.00e+00 (±0.00e+00)} & 5.98e-01 (±2.73e-02) & 6.34e-01 (±1.12e-02) & \textbf{1.00e+00 (±0.00e+00)} & \textbf{1.00e+00 (±0.00e+00)} \\
 MMF14     & \textbf{1.00e+00 (±0.00e+00)} & 5.85e-01 (±2.95e-02) & 8.68e-01 (±1.14e-02) & 9.53e-01 (±9.74e-02)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MMF15     & \textbf{1.00e+00 (±0.00e+00)} & 5.75e-01 (±1.65e-02) & 8.62e-01 (±8.55e-03) & \textbf{1.00e+00 (±0.00e+00)} & \textbf{1.00e+00 (±0.00e+00)} \\
 OmniTest  & \textbf{1.00e+00 (±0.00e+00)} & 5.69e-01 (±1.49e-02) & 7.27e-01 (±1.02e-02) & 7.42e-01 (±2.00e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SSUF1     & \textbf{1.00e+00 (±0.00e+00)} & 5.44e-01 (±2.30e-02) & 7.85e-01 (±5.97e-03) & 5.50e-01 (±9.74e-02)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SSUF3     & \textbf{1.00e+00 (±0.00e+00)} & 7.00e-01 (±3.56e-02) & 5.00e-01 (±7.07e-03) & 8.59e-01 (±1.31e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SymPart1  & \textbf{1.00e+00 (±0.00e+00)} & 5.93e-01 (±3.50e-02) & 6.87e-01 (±1.03e-02) & 6.87e-01 (±2.58e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SymPart2  & \textbf{1.00e+00 (±0.00e+00)} & 6.10e-01 (±3.49e-02) & 5.68e-01 (±1.28e-02) & 7.91e-01 (±1.08e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 SymPart3  & \textbf{1.00e+00 (±0.00e+00)} & 6.01e-01 (±1.78e-02) & 5.33e-01 (±1.34e-02) & 8.50e-01 (±1.30e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 TwoOnOne  & \textbf{1.00e+00 (±0.00e+00)} & 5.94e-01 (±1.71e-02) & 7.44e-01 (±9.55e-03) & 8.28e-01 (±8.67e-02)          & \textbf{1.00e+00 (±0.00e+00)} \\
\hline
\end{tabular}
\caption{Results for Smoothness indicator}
\label{tab:res_smooth}
\end{table*}

==> sections/tables-per-indicator.tex <==


%
%
% OLD FULL TABLE INCLUDING SET-BEZEA
%
%
\begin{comment}
\begin{table*}
\centering
\caption{Results (avg. ($\pm$ st.dev.)) per problem and algorithm over 31 runs, bold identifies best result with statistical significance (Wilcoxon rank-sum test with $\alpha = 0.05$ and Holm-Bonferroni correction).}
\label{tab:res_hv}
\scriptsize
\begin{tabular}{l|l|lllll}
\hline
  & Problem   & MM-BezEA                      & Set-BezEA                    & MO-HillVallEA                 & MO\_Ring\_PSO\_SCD               & MO-RV-GOMEA                   \\
\hline
 \multirow{11}{*}{\rotatebox[origin=c]{90}{~\large{HV}}} & MinDist   & \textbf{1.17e+2 (±9.43e-5)} & \textbf{1.17e+2 (±3.02e-4)} & 1.17e+2 (±1.62e-2)          & 1.17e+2 (±5.95e-3)          & 1.17e+2 (±1.36e-3)           \\
 & OmniTest  & \textbf{8.48e+0 (±2.18e-6)} & 8.43e+0 (±2.34e-1)           & 8.47e+0 (±1.96e-3)          & 8.47e+0 (±7.34e-4)          & 8.47e+0 (±4.82e-4)          \\
 & Sympart 1  & \textbf{1.17e+2 (±2.16e-5)} & 1.16e+2 (±1.67e+0)          & 1.17e+2 (±1.42e-2)          & 1.17e+2 (±7.64e-3)          & 1.17e+2 (±1.30e-3)          \\
 & Sympart 2  & \textbf{1.17e+2 (±2.91e-5)} & 1.15e+2 (±1.97e+0)          & 1.17e+2 (±7.77e-3)          & 1.17e+2 (±8.75e-3)          & 1.17e+2 (±4.47e-3)          \\
 & Sympart 3  & \textbf{1.17e+2 (±9.61e-5)} & 1.16e+2 (±1.76e+0)          & 1.17e+2 (±1.61e-2)          & 1.17e+2 (±9.21e-3)          & 1.17e+2 (±4.91e-3)          \\
 & TwoOnOne  & 1.13e+2 (±1.33e-4)          & 1.13e+2 (±9.27e-4)          & 1.13e+2 (±2.39e-4)          & \textbf{1.13e+2 (±1.82e-4)} & 1.13e+2 (±1.10e-4)          \\
 & MMF 1     & 6.04e-1 (±3.86e-2)          & 6.29e-1 (±5.63e-2)          & \textbf{8.05e-1 (±2.37e-4)} & \textbf{8.05e-1 (±8.69e-5)} & \textbf{8.05e-1 (±6.60e-5)} \\
 & MMF 2     & 6.34e-1 (±2.01e-4)          & 5.88e-1 (±9.42e-02)          & 8.04e-1 (±6.90e-4)          & 8.04e-1 (±9.59e-4)          & \textbf{8.05e-1 (±1.75e-4)} \\
 & MMF 12     & 1.78e+0 (±2.02e-6)          & 1.38e+0 (±2.02e-1)          & 2.06e+0 (±2.57e-3)          & 2.06e+0 (±2.05e-3)          & \textbf{2.06e+0 (±1.49e-4)} \\
 & MMF 14     & 5.63e+0 (±1.33e-5)          & 5.63e+0 (±6.40e-3)          & \textbf{5.63e+0 (±7.26e-4)} & 5.63e+0 (±1.92e-3)          & 5.63e+0 (±2.23e-4)          \\
 & MMF 15     & 5.56e+0 (±2.03e-2)          & 5.56e+0 (±4.47e-3)          & \textbf{5.57e+0 (±6.52e-4)} & 5.56e+0 (±1.54e-3)          & \textbf{5.57e+0 (±1.79e-4)} \\
\hline
%  Indicator & Problem   & MM-BezEA                      & MO-HillVallEA                 & MO\_Ring\_PSO\_SCD               & MO-RV-GOMEA          & Set-BezEA                    \\
%\hline
  \multirow{11}{*}{\rotatebox[origin=c]{90}{~\large{PSP}}} &MinDist   & \textbf{3.26e+2 (±7.31e+1)} & \textbf{3.77e+2 (±9.41e+1)} & 5.02e+1 (±2.74e+0)          & 6.97e+1 (±6.73e+0)          & 1.21e+0 (±1.65e+0) \\
  & OmniTest  & \textbf{2.36e+2 (±8.81e+1)} & 1.71e-2 (±3.34e-2)          & 7.13e+1 (±2.76e+0)          & 6.90e+1 (±9.56e+0)          & 1.36e-1 (±2.43e-1) \\
 &Sympart 1  & \textbf{2.67e+2 (±1.21e+2)} & 1.22e-3 (±2.89e-3)          & 3.56e+1 (±1.57e+0)          & 2.79e+1 (±3.69e+0)          & 1.16e-2 (±2.70e-2) \\
 &Sympart 2  & \textbf{3.09e+2 (±8.46e+1)} & 2.76e-4 (±3.54e-4)          & 3.60e+1 (±7.42e-1)          & 2.38e+1 (±2.46e+0)          & 1.02e-2 (±1.71e-2) \\
 &Sympart 3  & 6.41e+1 (±7.77e+1)          & 1.27e-3 (±2.17e-3)          & \textbf{4.33e+1 (±2.10e+0)} & 2.64e+1 (±5.62e+0)          & 8.09e-3 (±1.33e-2) \\
 &TwoOnOne  & \textbf{3.04e+2 (±2.18e+2)} & \textbf{2.69e+2 (±1.15e+2)} & 4.50e+1 (±7.21e-1)          & 2.45e+1 (±1.03e+1)          & 2.68e+0 (±1.11e+0) \\
 &MMF 1     & 7.22e+0 (±2.41e+0)          & 4.56e-1 (±3.55e-1)          & 3.17e+1 (±6.84e-1)          & \textbf{3.80e+1 (±6.79e+0)} & 1.02e+0 (±2.89e-1) \\
 &MMF 2     & 4.00e+0 (±2.49e+0)          & 4.29e-2 (±5.23e-2)          & \textbf{1.17e+2 (±1.21e+1)} & 5.04e+1 (±1.51e+1)          & 2.18e+0 (±1.41e+0) \\
 &MMF 12     & \textbf{2.42e+1 (±7.72e+0)} & 4.83e-1 (±6.81e-1)          & 1.94e+1 (±6.46e+0)          & 1.53e+1 (±1.46e-1)          & 8.67e+0 (±1.36e+0) \\
 &MMF 14     & \textbf{2.68e+3 (±4.82e+2)} & 1.72e+3 (±1.60e+3)          & 3.70e+2 (±1.03e+1)          & 2.31e+2 (±2.16e+1)          & 1.08e+0 (±2.84e+0) \\
 &MMF 15     & \textbf{2.73e+2 (±4.17e+1)} & 2.96e+2 (±1.41e+2)          & 2.65e+2 (±4.58e+0)          & 2.44e+2 (±7.25e+0)          & 2.24e+1 (±1.40e-2) \\
\hline
%  Indicator & Problem   & MM-BezEA                      & MO-HillVallEA        & MO\_Ring\_PSO\_SCD      & MO-RV-GOMEA                   & Set-BezEA                    \\
%\hline
  \multirow{11}{*}{\rotatebox[origin=c]{90}{~\large{Smoothness}}} & MinDist   & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 8.09e-1 (±3.70e-2) & 7.63e-1 (±5.91e-3) & 8.94e-1 (±1.81e-1)          \\
  & OmniTest   & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 9.23e-1 (±5.65e-3) & 7.28e-1 (±9.76e-3) & 7.16e-1 (±1.96e-1)           \\
 & Sympart 1  & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 8.76e-1 (±2.52e-2) & 6.84e-1 (±9.76e-3) & 7.01e-1 (±2.09e-1)          \\
 & Sympart 2  & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 8.78e-1 (±2.14e-2) & 5.73e-1 (±9.30e-3) & 7.87e-1 (±1.68e-1)          \\
 & Sympart 3  & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 8.70e-1 (±3.10e-2) & 5.29e-1 (±1.18e-2) & 8.30e-1 (±1.92e-1)          \\
 & TwoOnOne   & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 7.77e-1 (±1.21e-2) & 7.47e-1 (±9.36e-3) & 7.51e-1 (±1.59e-1)          \\
 & MMF 1      & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 9.01e-1 (±3.98e-2) & 7.82e-1 (±8.49e-3) & 5.86e-1 (±9.13e-2)          \\
 & MMF 2      & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 9.38e-1 (±1.26e-2) & 5.01e-1 (±8.92e-3) & 8.46e-1 (±1.60e-1)          \\
 & MMF 12     & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 8.35e-1 (±2.73e-2) & 6.35e-1 (±9.86e-3) & \textbf{1.00e+0 (±0.00e+0)} \\
 & MMF 14     & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 9.31e-1 (±1.17e-2) & 8.71e-1 (±1.11e-2) & 9.62e-1 (±1.05e-1)          \\
 & MMF 15     & \textbf{1.00e+0 (±0.00e+0)} & \textbf{1.00e+0 (±0.00e+0)} & 9.19e-1 (±1.43e-2) & 8.63e-1 (±8.54e-3) & \textbf{1.00e+0 (±0.00e+0)} \\
\hline
\end{tabular}
\vspace{-10pt}
\end{table*}
\end{comment}

==> sections/tables-per-problem.tex <==
\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & 1.18e+02 (±6.26e-08)          & \textbf{1.70e-01 (±1.30e-05)} & \textbf{9.27e-04 (±2.92e-06)} & \textbf{1.06e+03 (±1.90e+01)} & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & 1.18e+02 (±4.51e-03)          & 1.93e-01 (±4.71e-03)          & 2.08e-02 (±1.12e-03)          & 4.81e+01 (±2.56e+00)          & 5.98e-01 (±2.12e-02)          \\
 MO-RV-GOMEA   & 1.18e+02 (±1.01e-03)          & 1.94e-01 (±2.44e-04)          & 1.33e+00 (±8.55e-01)          & 1.49e+00 (±1.96e+00)          & 9.24e-01 (±1.01e-01)          \\
 Sets-BezEA    & 1.18e+02 (±3.48e-04)          & \textbf{1.71e-01 (±3.29e-04)} & 2.10e-03 (±2.15e-03)          & 7.38e+02 (±3.30e+02)          & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & \textbf{1.18e+02 (±5.77e-03)} & 1.80e-01 (±1.17e-03)          & 5.13e-01 (±5.13e-01)          & 1.76e+00 (±1.38e+00)          & 9.36e-01 (±8.38e-02)          \\
\hline
\end{tabular}

\caption{Results on MinDist}
\label{tab:mindist}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & 9.55e-01 (±4.14e-10)          & 4.44e-02 (±2.03e-06)          & \textbf{8.93e-02 (±1.25e-01)} & \textbf{5.09e+01 (±4.04e+01)} & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & 9.52e-01 (±2.77e-04)          & 5.18e-02 (±9.02e-04)          & \textbf{1.77e-02 (±1.26e-03)} & \textbf{5.66e+01 (±3.50e+00)} & 5.62e-01 (±2.04e-02)          \\
 MO-RV-GOMEA   & 9.51e-01 (±1.01e-04)          & 5.25e-02 (±4.34e-04)          & 1.42e+00 (±4.09e-01)          & 2.37e-01 (±3.82e-01)          & 7.53e-01 (±1.81e-01)          \\
 Sets-BezEA    & 9.55e-01 (±4.61e-05)          & 4.45e-02 (±4.95e-04)          & 1.68e+00 (±2.05e-01)          & 2.11e-02 (±4.60e-02)          & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & \textbf{9.56e-01 (±9.00e-05)} & \textbf{4.40e-02 (±3.40e-04)} & 1.98e+00 (±7.75e-04)          & 3.16e-05 (±5.98e-07)          & 9.98e-01 (±2.50e-03)          \\
\hline
\end{tabular}

\caption{Results on OmniTest d = 2}
\label{tab:omnitest_2}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & 1.18e+02 (±3.40e-08)          & \textbf{1.70e-01 (±1.28e-05)} & \textbf{1.08e-01 (±2.85e-01)} & \textbf{7.02e+02 (±5.33e+02)} & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & 1.18e+02 (±7.74e-03)          & 1.95e-01 (±2.42e-03)          & \textbf{2.78e-02 (±5.70e-04)} & 3.60e+01 (±7.32e-01)          & 5.82e-01 (±3.76e-02)          \\
 MO-RV-GOMEA   & 1.18e+02 (±9.74e-04)          & 1.93e-01 (±2.86e-04)          & 7.71e+00 (±2.15e+00)          & 6.82e-03 (±2.05e-02)          & 7.14e-01 (±1.66e-01)          \\
 Sets-BezEA    & 1.15e+02 (±2.27e+00)          & 2.42e-01 (±7.28e-02)          & 9.22e+00 (±8.62e-01)          & 8.45e-04 (±2.29e-03)          & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & \textbf{1.18e+02 (±5.57e-03)} & 1.78e-01 (±1.50e-03)          & 1.02e+01 (±1.09e-03)          & 1.17e-09 (±1.65e-09)          & 9.99e-01 (±8.46e-04)          \\
\hline
\end{tabular}

\caption{Results on SymPart1}
\label{tab:SymPart1}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & \textbf{1.18e+02 (±2.83e-08)} & \textbf{1.70e-01 (±9.65e-06)} & \textbf{2.06e-01 (±3.96e-01)} & \textbf{7.89e+02 (±5.15e+02)} & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & 1.18e+02 (±7.66e-03)          & 1.96e-01 (±3.53e-03)          & \textbf{2.83e-02 (±3.15e-03)} & 3.56e+01 (±3.12e+00)          & 5.79e-01 (±2.65e-02)          \\
 MO-RV-GOMEA   & 1.18e+02 (±1.58e-03)          & 1.91e-01 (±3.36e-03)          & 6.41e+00 (±1.51e+00)          & 1.55e-02 (±2.02e-02)          & 7.60e-01 (±1.15e-01)          \\
 Sets-BezEA    & \textbf{1.17e+02 (±1.42e+00)} & 1.86e-01 (±4.51e-02)          & 8.57e+00 (±6.53e-01)          & 5.01e-04 (±3.69e-04)          & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & \textbf{1.18e+02 (±3.59e-02)} & 1.81e-01 (±7.05e-03)          & 1.02e+01 (±1.62e-03)          & 4.51e-07 (±4.60e-09)          & 9.99e-01 (±1.26e-03)          \\
\hline
\end{tabular}

\caption{Results on SymPart2}
\label{tab:SymPart2}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & \textbf{1.18e+02 (±2.56e-07)} & \textbf{1.70e-01 (±1.78e-05)} & 9.64e-01 (±8.60e-01)          & 2.03e+01 (±5.63e+01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & 1.18e+02 (±8.56e-03)          & 1.95e-01 (±1.99e-03)          & \textbf{9.81e-02 (±2.16e-01)} & \textbf{3.83e+01 (±1.54e+01)} & 6.07e-01 (±3.61e-02)          \\
 MO-RV-GOMEA   & 1.18e+02 (±1.95e-03)          & 1.91e-01 (±3.90e-03)          & 6.46e+00 (±2.41e+00)          & 1.43e-02 (±2.23e-02)          & 8.49e-01 (±1.53e-01)          \\
 Sets-BezEA    & 1.18e+02 (±1.03e-01)          & 1.75e-01 (±1.05e-02)          & 7.85e+00 (±1.35e+00)          & 1.11e-03 (±7.09e-04)          & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & 1.18e+02 (±7.98e-02)          & 1.83e-01 (±1.40e-02)          & 8.91e+00 (±1.63e+00)          & 2.08e-04 (±4.28e-04)          & 9.93e-01 (±8.57e-03)          \\
\hline
\end{tabular}

\caption{Results on SymPart3}
\label{tab:SymPart3}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & 1.13e+02 (±9.03e-08)          & 3.87e-02 (±4.14e-06)          & 5.18e-03 (±4.83e-03)          & 2.57e+02 (±7.08e+01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & \textbf{1.13e+02 (±5.50e-05)} & 3.89e-02 (±1.29e-04)          & 2.21e-02 (±2.46e-04)          & 4.51e+01 (±4.77e-01)          & 5.95e-01 (±2.90e-02)          \\
 MO-RV-GOMEA   & \textbf{1.13e+02 (±5.29e-05)} & 3.90e-02 (±4.13e-05)          & 1.97e-01 (±3.01e-02)          & 3.48e+00 (±1.24e+00)          & 8.34e-01 (±1.14e-01)          \\
 Sets-BezEA    & 1.13e+02 (±6.48e-03)          & 3.90e-02 (±5.88e-04)          & \textbf{5.59e-02 (±1.58e-01)} & \textbf{2.72e+02 (±9.70e+01)} & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & 1.13e+02 (±2.58e-04)          & \textbf{3.81e-02 (±5.95e-04)} & 6.03e-01 (±1.48e-03)          & 1.03e-01 (±2.90e-04)          & 9.99e-01 (±1.08e-03)          \\
\hline
\end{tabular}

\caption{Results on TwoOnOne}
\label{tab:TwoOnOne}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & 5.99e-01 (±8.08e-03)          & 2.82e-01 (±3.06e-02)          & 1.51e-01 (±5.82e-02)          & 5.52e+00 (±2.03e+00)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & \textbf{8.23e-01 (±2.33e-04)} & \textbf{3.80e-02 (±3.78e-04)} & \textbf{3.19e-02 (±8.63e-04)} & \textbf{3.14e+01 (±8.59e-01)} & 5.35e-01 (±1.09e-02)          \\
 MO-RV-GOMEA   & \textbf{8.23e-01 (±1.45e-04)} & 3.85e-02 (±6.09e-04)          & 3.47e-01 (±2.52e-02)          & 1.87e+00 (±6.41e-01)          & 5.56e-01 (±4.25e-02)          \\
 Sets-BezEA    & 6.40e-01 (±4.10e-02)          & 2.38e-01 (±3.59e-02)          & 3.88e-01 (±1.07e-01)          & 3.36e-01 (±2.74e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & 8.06e-01 (±9.63e-03)          & 5.09e-02 (±7.44e-03)          & 4.06e-01 (±7.88e-02)          & 8.67e-01 (±6.18e-01)          & 6.51e-01 (±1.31e-01)          \\
\hline
\end{tabular}

\caption{Results on MMF1 (SSUF1)}
\label{tab:SSUF1}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & 6.38e-01 (±1.32e-09)          & 1.86e-01 (±8.48e-07)          & 2.97e-01 (±1.21e-01)          & 1.72e+00 (±2.25e+00)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & \textbf{8.23e-01 (±7.24e-04)} & \textbf{4.38e-02 (±1.32e-03)} & \textbf{1.02e-02 (±7.03e-04)} & \textbf{9.85e+01 (±6.61e+00)} & 6.82e-01 (±3.37e-02)          \\
 MO-RV-GOMEA   & \textbf{8.23e-01 (±3.32e-04)} & 4.52e-02 (±9.52e-04)          & 2.05e-01 (±8.98e-02)          & 3.64e+00 (±2.07e+00)          & 8.87e-01 (±1.23e-01)          \\
 Sets-BezEA    & 6.30e-01 (±5.09e-02)          & 1.77e-01 (±3.26e-02)          & 4.07e-01 (±1.28e-01)          & 1.35e-01 (±1.16e-01)          & \textbf{9.50e-01 (±1.50e-01)} \\
 UHV-GOMEA     & \textbf{7.43e-01 (±9.87e-02)} & 8.86e-02 (±5.62e-02)          & 3.59e-01 (±7.32e-02)          & 4.20e-01 (±1.99e-01)          & 8.47e-01 (±2.53e-01)          \\
\hline
\end{tabular}

\caption{Results on MMF2 (SSUF3)}
\label{tab:SSUF3}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & 1.77e+00 (±3.13e-02)          & 4.03e-01 (±1.56e-01)          & 6.12e-02 (±1.04e-02)          & 9.59e+00 (±4.76e+00)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & 2.07e+00 (±6.49e-04)          & 2.90e-01 (±1.73e-03)          & \textbf{5.13e-02 (±1.15e-03)} & \textbf{1.00e+01 (±2.22e-01)} & 5.95e-01 (±1.75e-02)          \\
 MO-RV-GOMEA   & 2.07e+00 (±1.66e-04)          & 2.90e-01 (±9.72e-05)          & 7.42e-02 (±3.51e-05)          & 6.89e+00 (±4.43e-03)          & \textbf{1.00e+00 (±0.00e+00)} \\
 Sets-BezEA    & 1.72e+00 (±1.62e-01)          & 3.31e-01 (±1.66e-02)          & 2.25e-01 (±3.55e-02)          & 3.26e-01 (±6.34e-01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & \textbf{2.07e+00 (±1.96e-03)} & \textbf{2.84e-01 (±5.49e-03)} & 7.28e-02 (±1.12e-03)          & 7.07e+00 (±1.04e-01)          & 1.00e+00 (±6.43e-05)          \\
\hline
\end{tabular}

\caption{Results on MMF12}
\label{tab:MMF12}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & 5.70e+00 (±1.05e-08)          & \textbf{8.72e-02 (±5.78e-10)} & 2.51e-04 (±8.27e-07)          & 3.98e+03 (±1.31e+01)          & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & \textbf{5.71e+00 (±2.92e-04)} & 9.92e-02 (±3.24e-03)          & 2.71e-03 (±7.00e-05)          & 3.69e+02 (±9.31e+00)          & 5.84e-01 (±2.48e-02)          \\
 MO-RV-GOMEA   & 5.71e+00 (±5.08e-05)          & 9.82e-02 (±1.19e-04)          & 2.27e-01 (±7.86e-02)          & 2.87e+00 (±5.73e+00)          & 9.27e-01 (±1.47e-01)          \\
 Sets-BezEA    & 5.70e+00 (±2.24e-13)          & 8.72e-02 (±1.77e-15)          & \textbf{2.50e-04 (±1.96e-10)} & \textbf{4.00e+03 (±3.17e-03)} & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & 5.71e+00 (±6.52e-03)          & 1.03e-01 (±3.69e-03)          & 1.63e-01 (±6.25e-02)          & 6.35e+00 (±3.85e+00)          & 8.96e-01 (±1.04e-01)          \\
\hline
\end{tabular}

\caption{Results on MMF14}
\label{tab:MMF14}
\end{table*}

\begin{table*}[h]
%\footnotesize
\small

\begin{tabular}{llllll}
\hline
 Method        & HV                            & IGDF                          & IGDX                          & PSP                           & Smoothness                    \\
\hline
 MM-BezEA      & 5.63e+00 (±2.42e-08)          & \textbf{8.81e-02 (±1.03e-09)} & \textbf{3.50e-03 (±7.10e-06)} & \textbf{2.86e+02 (±5.79e-01)} & \textbf{1.00e+00 (±0.00e+00)} \\
 MO-HillVallEA & 5.64e+00 (±1.36e-04)          & 1.01e-01 (±3.98e-03)          & 3.78e-03 (±7.92e-05)          & 2.65e+02 (±5.55e+00)          & 5.88e-01 (±3.02e-02)          \\
 MO-RV-GOMEA   & 5.64e+00 (±5.93e-05)          & 9.92e-02 (±1.21e-04)          & 3.17e-02 (±4.07e-05)          & 3.15e+01 (±4.05e-02)          & \textbf{1.00e+00 (±0.00e+00)} \\
 Sets-BezEA    & 5.63e+00 (±2.14e-11)          & 8.81e-02 (±1.96e-14)          & \textbf{3.50e-03 (±1.41e-07)} & \textbf{2.86e+02 (±1.15e-02)} & \textbf{1.00e+00 (±0.00e+00)} \\
 UHV-GOMEA     & \textbf{5.65e+00 (±5.67e-03)} & 1.04e-01 (±3.33e-03)          & 3.31e-02 (±1.01e-03)          & 3.02e+01 (±8.59e-01)          & 1.00e+00 (±3.96e-04)          \\
\hline
\end{tabular}

\caption{Results on MMF15}
\label{tab:MMF15}
\end{table*}
